GTA: Gated Toxicity Avoidance for LM Performance Preservation

Caution: This paper includes offensive words that could potentially cause unpleasantness. The fast-paced evolution of generative language models such as GPT-4 has demonstrated outstanding results in various NLP generation tasks. However, due to the potential generation of offensive words related to race or gender, various Controllable Text Generation (CTG) methods have been proposed to mitigate the occurrence of harmful words. However, existing CTG methods not only reduce toxicity but also negatively impact several aspects of the language model's generation performance, including topic consistency, grammar, and perplexity. This paper explores the limitations of previous methods and introduces a novel solution in the form of a simple Gated Toxicity Avoidance (GTA) that can be applied to any CTG method. We also evaluate the effectiveness of the proposed GTA by comparing it with state-of-the-art CTG methods across various datasets. Our findings reveal that gated toxicity avoidance efficiently achieves comparable levels of toxicity reduction to the original CTG methods while preserving the generation performance of the language model.

==> 0_rebuttal.tex <==
---------------------------------
@@@ Reviewer 4a3Y

Thank you for your detailed and insightful review.
Here are the comments on your review.
1 & 2) Novelty: The novelty of our work is an analysis of existing detoxifiers - detoxifiers decrease toxicity and also decrease LM performance - and our gated detoxifier can resolve the problems. With the marginal toxicity sacrifice (0.04 in PPLM, 0.00 in GeDi and DExperts), the gated detoxifier gains LM generation performance (topic preserving, grammar, and perplexity).


3) Confusing term 'detoxifier': Our term `detoxifier' is used for `guided decoder' of LM for non-toxic text generation. We picked a detoxifier from the previous detoxification studies [2020 Krause, Ben et al, 2022 Gu, Yuxuan, et al], but we agree that the term is confusing. We will clarify our task and change `detoxifier' to `guided decoder' for the camera-ready version.

 

Q. Is there any particular reason that you did not include the SOTA detoxifier, ParaDetox?

A. The proposed gated detoxifier is the guided decoder which can be applied to the CTG method, whereas its applicability to the text style transfer task is limited. Instead, we selected the state-of-the-art CTG method, DisCup, proposed in 2022. However, through a straightforward experiment, we also observed ParaDetox encountering challenges in text style transfer. Leveraging a toxic classifier, we curated a subset of 628 toxic samples from the emotion dataset. Then we attempted to transform these samples into non-toxic using ParaDetox. We evaluate the detoxified texts using the emotion classifier. We were able to observe variations in topic accuracy following detoxification, depending on the topic. The performance degradation (avg. -13.49\%) also occurred in the ParaDetox. We used emotion and toxicity classifier which also used in the paper. 

The obtained results are as follows:
- anger: 100.0 -> 57.17\% accuracy, 146 samples
- fear: 100.0 -> 84.85\% accuracy, 56 samples
- joy: 100.0 -> 96.36\% accuracy, 106 samples
- love: 100.0 -> 90.91\% accuracy, 50 samples
- sadness: 100.0 -> 89.79\% accuracy, 255 samples
- surprise: 100.0 -> 100\% accuracy, 16 samples

%A. Thanks to your suggestion, and we validated our method with ParaDetox. The gated detoxifier can be applied to the CTG method, whereas its applicability to the text style transfer task is limited. Despite efforts to explore potential application for applying the gating method to ParaDetox, we could not find a suitable approach. Even attempting to integrate the ParaDetox during the gated detoxifier process when toxic tokens are encountered did not yield favorable outcomes. Instead, we selected the state-of-the-art CTG method, DisCup, proposed in 2022.

%However, through a straightforward experiment, we also observed ParaDetox encountering challenges in text style transfer. Leveraging a toxic classifier, we curated a subset of 628 toxic samples from the emotion dataset. Then we attempted to transform these samples into non-toxic using ParaDetox. We evaluate the detoxified texts using the emotion classifier. We were able to observe variations in topic accuracy following detoxification, depending on the topic. The performance degradation also occurred in the ParaDetox. We used emotion and toxicity classifier which also used in the paper. 

%The obtained results are as follows:
%- anger: 100.0 -> 57.17\% accuracy, 146 samples
%- fear: 100.0 -> 84.85\% accuracy, 56 samples
%- joy: 100.0 -> 96.36\% accuracy, 106 samples
%- love: 100.0 -> 90.91\% accuracy, 50 samples
%- sadness: 100.0 -> 89.79\% accuracy, 255 samples
%- surprise: 100.0 -> 100\% accuracy, 16 samples


Thank you for pointing out typo errors. We will conduct multiple proof-reading before submitting the final version.


[1] Krause, Ben, et al. ``Gedi: Generative discriminator guided sequence generation." arXiv preprint arXiv:2009.06367 (2020).
[2] Gu, Yuxuan, et al. ``Improving controllable text generation with position-aware weighted decoding." Findings of the Association for Computational Linguistics: ACL 2022. 2022.
[3] Zhang, Hanqing, and Dawei Song. ``DisCup: Discriminator cooperative unlikelihood prompt-tuning for controllable text generation." arXiv preprint arXiv:2210.09551 (2022).


- 

---------------------------------
@@@ Reviewer 9wix


1) Instruction-tuned & 2) Reinforcement Learning from Human Feedback (RLHF):

To focus on the toxicity in the paper, we select CTG methods for the baselines. The objectives of instruction-tuned and RLHF are toxicity (harmfulness) and helpfulness. Thank you for your constructive comments, and we validate toxicity on LLaMA (meta-llama/Llama-2-7b-chat-hf [1] in the huggingface). This is a instruction-tuned model with Reinforcement Learning from Human Feedback (RLHF). We utilized the following prompts to generate 6,000 tweets containing six different emotions. The emotion and toxic classifiers are same as used in the paper. 

We also observed that CTG methods show the better performance on toxicity. The average toxicity of LLaMA is 0.67\% (anger: 2.20\%, fear: 1.10\%, joy: 0.20\%, love: 0.10\%, sadness: 0.20\%, and surprise: 0.20\%). When using the CTG method, we observed that GeDi yielded a remarkably low toxicity rate of 0.03\% on the GPT-2 (125M) model, while DExperts exhibited a similar low toxicity rate of 0.05\%. Given the substantial reduction in toxicity, the CTG technique proves to be highly valuable as a means to mitigate toxicity. We will supplement that modern RLHF models like LLaMA also encounter similar challenges.


%Thank you for your constructive comments, and we validate our model on LLaMA (meta-llama/Llama-2-7b-chat-hf [1] in the huggingface). This is a instruction-tuned model with Reinforcement Learning from Human Feedback (RLHF). We utilized the following prompts to generate 6,000 tweets containing six different emotions. The emotion and toxic classifiers are same as used in the paper.

%\begin{verbatim}
%emotions = ["anger", "sadness", "joy", "love", "fear", "surprise"]
%Prompt: Write a tweet where you feel like the author is in {emotion}
%\end{verbatim}

% \begin{table}[]
% \begin{tabular}{lll}
% \textbf{Emotion}  & \textbf{Topic Accuracy} & \textbf{Toxicity} \\
% \textbf{anger}    & 57.70\%                 & 2.20\%            \\
% \textbf{fear}     & 58.50\%                 & 1.10\%            \\
% \textbf{joy}      & 88.00\%                 & 0.20\%            \\
% \textbf{love}     & 13.30\%                 & 0.10\%            \\
% \textbf{sadness}  & 64.50\%                 & 0.20\%            \\
% \textbf{surprise} & 20.50\%                 & 0.20\%           
% \end{tabular}
% \end{table}

%The average toxicity stands at 0.67\%. When using the CTG method, we observed that GeDi yielded a remarkably low toxicity rate of 0.03\% on the GPT-2 (125M) model, while DExperts exhibited a similar low toxicity rate of 0.05\%. Given the substantial reduction in toxicity, the CTG technique proves to be highly valuable as a means to mitigate toxicity. We will supplement that modern RLHF models like LLaMA also encounter similar challenges.


3) Any overhead on top of a base LM is not preferred during the inference stage of decoding.
It is true that the CTG technique has performance overhead. This overhead was concerned significantly when deploying real-world service. In the light of these concerns, our methods decrease such overhead. The generation of toxic text poses substantial risks in practical service scenarios. Consequently, our work holds the potential to be applied in contexts where the generation of toxic content carries significant risks.


4) Significance of the results:
RQ1: GeDi seems to be at par with the base LM in terms of fluency as per the results in Table 1. The authors claim that GeDi hurts LM performance is therefore not convincing.
RQ2: While the gating scheme helps in improving the linguistic quality of PPLM and DExperts, GeDi doesn't seem to need the gating function for improving linguistic quality (Table 3).

RQ1 & RQ2: GeDi performance

On average, GeDi appears to be rather better on linguistic quality metrics. However, when looked at by topic, the results are different. Detoxifier's performance degradation occurs differently depending on the topic and metric. This table is the evaluation result of GPT-2, GeDi, and GeDi\_{gated} at small scale.

% ~(↑)} & \textbf{Toxicity~(↓)

Changes of GeDi's linguistic quality
- emotion topics: 88.31 -> 91.06 (+2.85\%p)
- sentiment topics: 88.22 -> 82.09 (-6.13\%p)

GeDi increases linguistic quality only in the emotion topics. The reason is that the texts in the emotion dataset are missing grammatical elements such as comma and apostrophe. On the other hand, in the sentiment dataset, the linguistic quality is rather greatly reduced. Sentiment has 2 topics, emotion has 6 topics. As a result, when micro-averaged, the difference in emotion is more prominent. We will add these qualitative results in the appendix.

 

Questions: 

Q.A) I could not find the architecture and training details of the gating function/model.

We will add the details of architecture and training information. We used the s-nlp/roberta\_toxicity\_classifier model, publicly available on Hugging Face, as our gating model. This model is trained for toxicity classification task. The dataset used for training is the merge of the English parts of the three datasets by Jigsaw (Jigsaw 2018, Jigsaw 2019, Jigsaw 2020), containing around 2 million examples. This model is fine-tuned RoBERTa[2] model for toxicity classification task. The dataset used for training are Jigsaw datasets (\href{https://www.kaggle.com/c/jigsaw-toxic-comment-classification-challenge}{Jigsaw 2018}, \href{https://www.kaggle.com/c/jigsaw-unintended-bias-in-toxicity-classification}{Jigsaw 2019}, \href{https://www.kaggle.com/c/jigsaw-multilingual-toxic-comment-classification}{Jigsaw 2020}), containing around 2 million examples. The classifiers perform closely on the test set of the first Jigsaw competition, reaching the AUC-ROC of 0.98 and F1-score of 0.76. Since this is not the model we trained, the training details are unknown.



Q.B) Line 480: Why is this the case? Why are toxicity classifiers less expensive than detoxifiers?

Our gated detoxifier is less expensive than the original detoxifiers. The total parameters of the gate model (gating network + toxicity classifiers) are 110M, but GeDi requires 355M parameters and DExperts requires 1550M parameters (it uses two 775M models). In addition, the probability of generating a toxic sentence in gpt-2 is only 1.85\%. Even within a sentence, few tokens are toxic. Therefore, the generation speed can be reduced compared to applying a detoxifier to every generation step.

%because the size of the gate model is much smaller. In a token generation, the original detoxifiers always adjust the probability of each token, but the gated detoxifier only adjusts the probability when the generated sentence is toxic. The gate model has 110M parameters, but GeDi requires 355M parameters and DExperts requires 1550M parameters (it uses two 775M models).


To clarify our method, we will change our paper title for the camera-ready version.

Thank you for pointing out typo errors. We will conduct multiple proof-reading before submitting the final version.


[1] Touvron, Hugo, et al. "Llama 2: Open foundation and fine-tuned chat models." arXiv preprint arXiv:2307.09288 (2023).
[2] Liu, Yinhan, et al. "Roberta: A robustly optimized bert pretraining approach." arXiv preprint arXiv:1907.11692 (2019).

---------------------------------
@@@ Reviewer Gtqh
Thank you for your detailed and insightful review. Here are the comments on your review.


1) Modern LLM:
Thank you for your comments, and we also validate our model on LLaMA (meta-llama/Llama-2-7b-chat-hf [1] in the huggingface). This is a instruction-tuned model with Reinforcement Learning from Human Feedback (RLHF). We have not tried applying gated detoxifier to modern LLM. We confirmed that toxicity is still a major issue in this model. We generated a total of 6000 short tweets which containing 6 emotions. Afterwards, we evaluated how accurate with emotion these tweets were and how toxic they were. For evaluation, the classifiers used in the paper were used.

- anger: 57.7\% accuracy, 2.2\% toxicity
- fear: 58.5\% accuracy, 1.1\% toxicity
- joy: 88\% accuracy, 0.2\% toxicity
- love: 13.3\% accuracy, 0.1\% toxicity
- sadness: 64.5\% accuracy, 0.2\% toxicity
- surprise: 20.5\% accuracy, 0.2\% toxicity

The average toxicity is 0.67\%. It can be seen that llama trained with RLHF still shows high toxicity in certain topics. Compared to GeDi's 0.03\% and DExperts' 0.05\%, that's a huge toxicity difference. Even with modern LLM, we can see that there is still a lot of room for improvement.

[1] Touvron, Hugo, et al. "Llama 2: Open foundation and fine-tuned chat models." arXiv preprint arXiv:2307.09288 (2023).


---------------------------------
@@@ Reviewer Byj4

Thank you for your detailed and insightful review. Here are the comments on your review.


1 & 3) Main contributions:

In order to commercialize the generative model, detoxification and subsequent performance degradation have received a lot of attention. However, it mainly focused on partial analysis - linguistic quality [1] or gender/regional/racial bias [2] -. To the best of our knowledge, this is the first analysis work of various aspects of LM performance degradation (topic preserving, grammar, and perplexity) of detoxification. We also conducted extensive experiments with four baselines (PPLM, GeDi, DExperts, and DisCup).
%On the other hand, research on topic preservation has not existed before. 


We analyze the performance degradation of existing detoxification methods, and we also propose a simple gated detoxifier that controls the detoxifier to lower the toxicity without sacrificing LM performance. In addition, the gated detoxifier significantly decreases the cost of original detoxifiers of the Controllable Text Generation (CTG) technique. Even though GeDi and DExperts show low toxicity, they have not been used in practice because of their inference time cost. This is the first approach that can significantly reduce the overhead of CTG techniques. 


%Our method is not intended to obtain better toxicity mitigation than existing detoxifiers. The goal is to control the detoxifier to lower the toxicity that the detoxifier can produce without sacrificing LM performance. We have been able to achieve that goal.

%The gated detoxifier significantly decreases the cost of detoxifiers of the CTG (Controllable Text Generation) technique. The one of the reason why CTG techniques such as GeDi and DExperts were not used in practice even though they can significantly lower toxicity is the overhead cost. We first proposed a method that can significantly reduce the overhead of CTG techniques. 

%The gated detoxifier is a very simple mechanism. However, its gain is huge, proposed for the first time. It is model-agnostic and easy to implement. Detoxifiers can be used more actively through the gating mechanism.

2) Technical details:

Q. Due to PPLM, GeDi, and DExperts being controllable generation models for detoxification, applying the gated detoxifier on top of them is easy to improve language quality (e.g., topic accuracy, grammar) while maintaining low toxicity. How about the performance for GPT-2 with the gated detoxifier?

We conducted an experiment which add a gate to GPT-2 without a detoxifier. When a toxic token is generated, sampling is performed again. This method had no performance difference from only using GPT-2. In the gated GPT-2, toxic tokens are continuously generated even if toxic tokens are resampled from one token to another because the context has a great influence on toxic text. Therefore, at that moment, the detoxifier must intervene and change the probability distribution.

Thanks for highlighting the typographical errors. We'll ensure several rounds of proofreading are done before the final submission.

[1] Gu, Yuxuan, et al. ``Improving controllable text generation with position-aware weighted decoding.`` Findings of the Association for Computational Linguistics: ACL 2022. 2022.
[2] Xu, Albert, et al. ``Detoxifying language models risks marginalizing minority voices.`` arXiv preprint arXiv:2104.06390 (2021).




==> __bak/4_methodsbak.tex <==
\com{here.....}

%\com{In this section, we first introduce why detoxifier degrade language model performance and propose our gated detoxfier.}

\subsection{Why detoxifier degrades language model performance?}
When training the detoxifier, it uses sequence-level labeled data, which assumes that all tokens in a sentence are toxic or not. Therefore, it not only avoids toxic word generation, but also avoids the generation of text with a similar distribution to toxic labeled data, and induces text to be generated with non-toxic labeled data. Because of this, detoxifiers avoid topics, tone, and expressions that often appear in toxic data and degrade performance. In order to preserve LM performance and lower toxicity, the influence of the detoxifier at an unnecessary moment must be minimized.

% Without loss of generality, we can formally define the weighted decoding detoxifiers as follows. 
Then, how can we minimize the influence of discriminators? In the proposed CTGs, the discriminator works at every generation step. That is, it also affects when LM generates non-toxic tokens. If the discriminator operates only when the LM creates a toxic token, it is possible to generate a non-toxic token while being topic-preserved.


\subsection{Ours: Gated Detoxifier}
We propose a gated detoxifer that selectively applies the detoxifier during the auto-regressive generation process. Gate model \(g(x)\) determines the operation of the detoxifier, and \(g(x)\)  is the pre-trained binary toxic classifier. \(g(x)\) returns 0 if the input string is toxic and 1 otherwise. When the token to be generated is toxic, the detoxifier is applied to change it to a non-toxic token. Formally, gated detoxifier for guided-decoding-based approaches~\cite{dathathri2019plug,krause2020gedi,Yang_2021,liu2021dexperts} is defined as

\begin{equation} \label{eq_gated_detoxifier_guided}
\begin{split}
p_{gated}(x_i|c) = p(x_i|X_{<i},c)p(c|X_{\leq i})^{g(X_{\leq i})}
\end{split}
\end{equation}

For prompt-tuning-based approaches~\cite{zhang2022discup}, It is defined as

\begin{equation} \label{eq_gated_detoxifier_prompt}
\begin{split}
p_{gated}(x_i|c) = p(x_i|X_{<i})p(X_i|[\hat{P};\hat{X}_{<i}])^{g(X_{\leq i})}
\end{split}
\end{equation}


The ultimate goal of Topic Preserving Detoxifier is for LM to generate topic-preserving and non-toxic text. Topic preservation can be evaluated as Topic Accuracy. This indicates how closely the generated text actually matches the topic when you ask the LM to generate text that match a given topic. Topic Accuracy is evaluated using a Topic Classifier model trained using a labeled dataset. The Topic Classifier calculates the probability that text is a topic. Toxicity can also be evaluated using a Toxicity Classifier trained with toxic labeled data. Our goal is that when LM receives topic c and generates a text, the generated text X shows high topic accuracy and low toxicity.

For the Gated Detoxifier to work, it needs to know about the next token to generate. When using the sampling, since the next token cannot be predicted with only the output distribution, it is necessary to actually sample it. Gated Detoxifier generates the next token by sampling without detoxifier, and then determines whether the token is toxic by using the gate model. If the tokens generated later and the previous sentences are determined to be toxic, a detoxifier is applied to the output distribution and then sampled again. Figure~\ref{fig:gate}

% \input{alg_pseudo}

%Toxic classifier
\textbf{Binary Toxic Classifier: Gate Model} The Gate Model to perform toxic classification has a transformer-based architecture and is trained by a toxic dataset. This model returns the probability of toxicity for a given text. If the probability is larger than threshold \(\theta\), detoxifier works, otherwise, it doesn't. In our experiments, we used 0.5 on both small scale and large scale. You can use a larger, better model to improve accuracy, or a smaller model to reduce inference cost.

% \textbf{Efficiency} Gated detoxifier seems to cost more because the cost of the gate model is added to the detoxifier. But in reality it is not. Because the probability of generating a toxic token is basically low, and if the Gate determines that it is non-toxic, the detoxifier is not called. Therefore, very little detoxifier overhead occurs, and mainly only gate model overhead occurs. However, since the overhead caused by the detoxifier is greater, the gated detoxifier can show a faster generation speed.

==> __bak/6_exp_resultbak.tex <==
\section{Experiments}
In this section, we will answer the following research questions:
\begin{itemize}
    \item{RQ1) Do detoxifiers reduce toxicity but degrade performance?}
    \item{RQ2) Can a gated detoxifier reduce toxicity, but preserve performance?}
    \item{RQ3) Does the performance degradation vary by topic?}
    \item{RQ4) Does the problem also occur on a larger scale? Is the solution robust to scale?}
    \item{RQ5) Efficiency: Is gated detoxifier more effective for inference than non-gated detoxifier?}
\end{itemize}

\com{
RQ1) Do detoxifiers degrade LM performance?
RQ2) Can gated detoxifier reduce toxicity without 
}


\subsection{RQ1: Detoxifier Degradation Effects}
\subsection{RQ2: Overall Performance of Gated Detoxifier}
\subsection{RQ3: Effectiveness of Topic}
\subsection{RQ4: Efficiency of Gated Detoxifier}

\subsection{RQ5: Detoxifier with Large-scale LM}
%Result analysis


\subsection{RQ6: Human Evaluation}
%human evaluation setting

%results



\subsection{Evaluation} 
For answering the research questions, we conduct automatic evaluation and human evaluation.

\subsubsection{Automatic Evaluation}
Automatic evaluation using the learned classifier is highly accurate and fast. We used 3 metrics to evaluate the generated text. Those are Topic Accuracy, Toxicity, Grammar. 

\textbf{Topic Accuracy} is a metric of how much text contains the given topic. We evaluated 13 topics. These topics are broadly divided into three groups.
\textbf{Sentiment} is a topic group that indicates a emotion of text to positive or negative. 
\textbf{Emotion} is also a topic group that indicates emotion of text. But It was divided into more detailed 6 topic(anger / sadness / fear / surprise / joy). 
\textbf{BBC News} is a topic group that indicates news article topic. It is divided into 5 topics(tech / sport / entertainment / politics / business). 

To evaluate these topics, we used a classifier based on the published transformer encoder. The sentiment classifier is a RoBERTa~\cite{liu2019roberta} model\footnote{\hyphenpenalty=100000 https://huggingface.co/VictorSanh/roberta-base-finetuned-yelp-polarity} which was finetuned with yelp-polarity\cite{zhangCharacterlevelConvolutionalNetworks2015} sentiment classification dataset. The emotion classifier is a BERT~\cite{devlin2018bert} model\footnote{\hyphenpenalty=100000 https://huggingface.co/bhadresh-savani/bert-base-uncased-emotion} which was finetuned with emotion classification dataset\cite{saravia-etal-2018-carer}. The BBC News classifier is a DistilBERT~\cite{sanh2019distilbert} model which was finetuned with bbc-news dataset\cite{yufeng_2018}.

\textbf{Toxicity} is a metric of how toxic the text is. We used Perplexity API\footnote{https://github.com/conversationai/perspectiveapi}, which is widely used to  
\textbf{Grammar} is a metric of how much texts are grammatically correct. It is a metric for evaluating the quality of text. 
\textbf{Perplexity(PPL)} is a metric used to evaluate how well a language model predicts a given sequence of words. A lower perplexity value indicates that the model is more confident and accurate, while a higher perplexity suggests more uncertainty and poorer. Perplexity was evaluated with the baseline LM that generated each text.


% 분량 없으면 appendix로 뺄거임.
% \subsubsection{Generation}
% 텍스트를 생성할 때 주제별로 다른 길이로 생성했다. sentiment는 32토큰, emotion은 64토큰, bbc-news는 128토큰을 생성했다. 이 값은 dataset의 평균 토큰길이를 측정한 값이다.
% bbc news 데이터셋은 평균 길이가 400토큰이었으나, 생성에 시간이 많이 걸리고 더 긴 텍스트를 생성해도 정확도가 증가하지 않아서 128을 최대 길이로 지정했다. 최대 길이에 도달하지 않더라도 early stopping이 가능했다. 
% 생성은 Top-k sampling과 Nucleus(Top-p) Sampling~\cite{holtzman2020curious}를 이용했으며 생성 파라미터로는 K=50, P=0.9 이다. 
% 텍스트는 topic마다 1000개씩 생성했다.


\subsubsection{Human Evaluation} 
Human evaluation is also commonly used to evaluate language model generation. However, because of the high cost, we only performed it at large-scale. 

We had humans evaluate three metrics of generated texts: Topic Accuracy, Toxicity, and Fluency. Topic accuracy was rated as 1 if the generated text matched the presented topic and 0 otherwise. Toxicity was evaluated as 1 if toxic contents were included and 0 otherwise. Fluency was rated on a 1(not fluency at all) - 5(very fluency) range. In order to reduce the bias of absolute evaluation, users were asked to review all samples before evaluation.

We evaluated the texts generated by the large-scale LM on 10 english experts. We used a total of five methods with a large-scale baseline LM, two SOTA detoxifiers, and two SOTA detoxifiers with gates. Each method generated 100 texts per topic. The evaluator randomly sampled two of them and evaluated them. Evaluators evaluated a total of 130 texts - 5 methods, 13 subjects, and 2 samples per subject. The evaluation took 35 minutes on average.
%
% 5.2 Detoxifier
%
%
%
\subsection{Detoxifier}
We tried to generate text using many detoxifiers. However, generating text on various topics from a large model was too costly. Therefore, first, experiments were performed using various detoxifiers in a small-scale LM, the best baseline was selected, and the experiment was performed on a large-scale.

\subsubsection{Small-scale Baseline}
In a small-scale experiment, we used traditional three detoxifiers - PPLM, DExperts, GeDi.
For using \textbf{PPLM}~\cite{dathathri2019plug}, we trained a classification head of each topic-generation LM. It was trained using published PPLM repository's code\footnote{https://github.com/uber-research/PPLM}.
For using \textbf{DExperts}, we used published large(775M)-scale toxicity expert and anti-expert in the paper. We used guide strength $\alpha$ to 0.5 and 1.0. Strength of 1.0 is enough to reduce toxicity. Larger strength degraded dramatically the generation quality.
For using \textbf{GeDi}, we used published 355M-scale toxicity CC-LM(Conditional-Controllable LM) in the paper. We used strength $\omega$ to 15 and 30. Larger strength also greatly degraded the generation quality.

small scale baseline LM is GPT-2 small(124M). However, it lacked the ability to generate texts match to the topic.
Therefore, we fine-tune the LM with 3 topic group datasets. Fine-tuned models generated better texts that matched the given topic. \ie Table~\ref{tab:topic_generation}, If a topic is given as a prompt, a related text is generated. 

% 우리는 3종류의 데이터셋을 이용하여 GPT2-small~\cite{radford2019language}을 파인튜닝해서 만들었다. 각 데이터셋은 텍스트와 텍스트의 topic이 라벨링되어있다. 
% sentiment topic generation을 위해서 yelp-polarity\cite{zhangCharacterlevelConvolutionalNetworks2015} 데이터셋을 LM에 파인튜닝했다. 
% Emotion topic generation을 위해 emotion\cite{saravia-etal-2018-carer} 데이터셋을 LM에 파인튜닝했다. 
% 마지막으로 bbc-news topic generation은 \cite{yufeng_2018} 데이터셋을 이용해서 LM에 파인튜닝했다. 
% 이렇게 3개의 데이터셋으로 3가지 파인튜닝된 모델을 만들었다. 이들은 총 13가지의 topic을 담은 문장을 생성할 수 있다. 이렇게 학습된 Topic Generation LM은 topic을 prompt로 제시하면 일치하는 문장을 생성한다(Table \ref{tab:topic_generation}).

% appendix로 보낼까..?
\input{tab_example}

\subsubsection{Large-scale Baseline}
In a large-scale experiment, We used 775M-scale GPT2-large~\cite{radford2019language} as a baseline LM. 
As a Baseline Detoxifier, we selected GeDi, best-performed in a small-scale experiment, and DisCup~\cite{zhang2022discup} - Large-scale SOTA. Unlike small-scale, we used In-context Learning to generate topic-matched texts. number of shot was different by topic. We used 10 shots for sentiment topics, 5 shots for bbc-news topic, 30 shots for emotion topics. Shots were randomly selected from topic dataset. Only non-toxic samples were used, and for sentiment and bbc-news topics, only up to 3 sentences of each sample were used.

\subsubsection{Gated Detoxifier}
For the Gate model, we used the RoBERTa model\footnote{\hyphenpenalty=100000 https://huggingface.co/s-nlp/roberta\_toxicity\_classifier} which was finetuned with JigSaw~\cite{jigsaw2018} toxic classification dataset. LM and Gate models use different tokenizers. For this reason, the token generated at each LM generation step was decoded with the LM tokenizer, then encoded using the Gate model tokenizer and used for Gate model inference. If we train a gate model using the same tokenizer, we can eliminate the decoding overhead.

Gate Threshold $\theta$ is used to determine whether the detoxifier works or not. In our experiments, we used 0.5 on both small scale and large scale. Even when a lower threshold was used, the difference was negligible.
%%
%% 5.3 Result Section
%%
%%
\section{Small-scale Result}
\subsection{Performance degrading of Detoxifier}

\input{tab_exp_small_result_test}


We found that detoxifiers reduce the toxicity but degrade the LM performances through automatic evaluation. This phenomenon varies depending on detoxifier, strength, and topic.

% PPLM
In the case of PPLM, the quality of the generated text was very low, and certain keywords were repeatedly generated in some topics. This phenomenon led to a phenomenon in which PPLM's accuracy skyrocketed in certain topics. This results in better average topic accuracy than DExperts.

% GeDi에 대한 내용
GeDi preserve grammar and perplexity well regardless of strength $\omega$. However, larger strength not only reduce toxicity but also degrade average topic accuracy. When strength is greater than 30, the generation quality is degraded significantly. GeDi is the overall best among the three detoxifiers, so we adopted it as a large scale detoxifier.

% DExperts에 대한 내용
DExperts significantly reduce grammar and perplexity. DExperts shows better performance at higher alpha(1.0). The reason for this phenomenon is maybe that the experts are 775M, which is much larger than the small baseline LM (124M), so that seems to have a good effect. When using smaller(124M) experts which we learned, DExperts degrade LM performance as the strength increased, as in GeDi. However, when the alpha value was greater than 1.0, poor quality text was generated.

\begin{figure}[t]
    \centering
    \small
    \includegraphics[width=\columnwidth]{image/exp_problem.png}
    \caption{The bottom bar chart shows the topic accuracy reduced by the detoxifier in \%p. The top line chart shows the toxicity (\%) of each method.}
    \label{fig:exp_problem}
\end{figure}


\subsection{Performance Preservation of Gated Detoxifier}

% \begin{figure}[t]
%     \centering
%     \small
%     \includegraphics[width=\columnwidth]{image/exp_gate_toxicity.png}
%     \caption{Toxicity Reduction of Gated Detoxifier}
%     \label{fig:exp_detox_toxicity}
% \end{figure}
% \begin{figure}[t]
%     \centering
%     \small
%     \includegraphics[width=\columnwidth]{image/exp_gate_topic.png}
%     \caption{Topic preserving of Gated Detoxifier}
%     \label{fig:exp_detox_topic}
% \end{figure}

We have shown through experiments that average topic accuracy, grammar, and perplexity can be preserved while toxicity is reduced when a gated detoxifier is used. These results are robust to detoxifiers, topics and strengths. Gated detoxifiers show slightly higher average toxicity than non-gated detoxifiers. This gap can be reduced by controlling the gate threshold $\theta$. The lower the threshold, the more frequently the detoxifier is used. It degrades the LM performance but reduce the average toxicity.

\begin{figure}[t]
    \centering
    \small
    \includegraphics[width=\columnwidth]{image/exp_toxicity_dist.png}
    \caption{Toxicity distribution of generated texts. The dotted line in the middle is 0.5.}
    \label{fig:exp_toxicity_dist}
\end{figure}

However, A high average toxicity is not a necessarily bad thing. In Figure~\ref{fig:exp_toxicity_dist}, in addition to high toxicity of 0.5 or higher, detoxifiers reduce distribution even in the "slightly toxic" score range between 0.1 and 0.5.
On the other hand, Gated Detoxifier shows a similar distribution to LM in the “slightly toxic” score range. In this distribution, there are texts that are not toxic but are negative, or deal with topics such as sexual or minority group(\ie{Table~\ref{tab:slightly_toxic_generation}}). The gated detoxifier reduces highly toxic expressions, while preserving the ability to generate slightly toxic(not actually toxic) text. This is why average toxicity is high, but performance is preserved.

% \include{tab_slightly_toxic_examples}

% gated detoxifier는 baseline과 유사하다 vs gated detoxifier는 non-gated detoxifier보다 좋다.

\subsection{Performance Analysis by Topic}

% \begin{figure*}[tbh]
%     \begin{subfigure}[h]{0.47\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{image/exp_detox_topic_acc.png}
%         \caption{Topic accuracy changes(↑)}
%         \label{fig:intro_toxicity}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.47\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{image/exp_detox_toxicity.png}
%         \caption{Average Toxicity(↓)}
%         \label{fig:concept_graph}
%     \end{subfigure}
    
%     \caption{Effect of Detoxifier(GeDi $\omega=30$), by topic. $\times$ is a Detoxifier, $\bigcirc
% $ is a Gated Detoxifier, $\Box$ and dotted line is baseline LM.}
% \end{figure*}

\begin{figure*}[tbh]
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\columnwidth]{image/exp_detox_topic_acc.png}
        \caption{Topic Accuracy(↑)}
        \label{fig:gedi_topic_acc}
    \end{subfigure}
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\columnwidth]{image/exp_detox_grammar.png}
        \caption{Grammar (↑)}
        \label{fig:concept_graph}
    \end{subfigure}    
    % \begin{subfigure}[t]{0.5\textwidth}
    %     \centering
    %     \includegraphics[width=\columnwidth]{image/exp_detox_toxicity.png}
    %     \caption{Toxicity(↓)}
    %     \label{fig:intro_toxicity}
    % \end{subfigure}
    % \begin{subfigure}[t]{0.5\columnwidth}
    %     \centering
    %     \includegraphics[width=\columnwidth]{image/exp_detox_ppl.png}
    %     \caption{Perplexity(↓)}
    %     \label{fig:concept_graph}
    % \end{subfigure}
    
    \caption{Effect of Detoxifier(GeDi $\omega=30$), by topic. $\times$ is a Detoxifier, $\bigcirc
$ is a Gated Detoxifier, $\Box$ and dotted line is baseline LM.}
\end{figure*}

We looked at the effect of detoxifiers on performance in detail by topic.

% Degradation이 topic 별로 다르다. GeDi를 보면
it can be seen that the performance degradation is different for each topic. In Figure~\ref{gedi_topic_acc}, GeDi seems to have a very small degradation in performance on average, but it showed a sharp degradation in accuracy in certain topics(anger, love, sadness) and no significant effect in other topics.

% Toxicity가 topic 별로 다르다.
Toxicity is different for each topic. Topics with high toxicity are anger (13.1\%) and sadness (7.8\%). LM without detoxifier showed toxicity of 2.48\% on average for all topics. This indicates that 2.48 texts contain toxic contents when 100 texts are generated. Except for emotion topics and negative topics, the remaining topics showed extremely low toxicity. High toxicity is related to degradation. For the anger and sadness topics, every detoxifier degrade the topic accuracy significantly.


% 어떤 detoxifier는 특정 topic accuracy를 증가시키기도 한다. 
In DExperts, on the other hand, positive topic accuracy increased and negative topic accuracy decreased. This means that there is a topic-specific bias depending on the detoxifier.


%
% Efficiency
%
%
\subsection{Efficiency of Detoxifier}
\begin{figure}[t]
    \centering
    \small
    \includegraphics[width=\columnwidth]{image/exp_eff_time.png}
    \caption{Time taken to generate 100 texts of 100 tokens length}
    \label{fig:exp_gated_detox_efficiency}
\end{figure}

% 빨라요
Gated Detoxifier not only preserve the LM performance, but also generate text more efficiently. It makes the LM generate much faster than the detoxifier without gate. To evaluate the time it took the detoxifier to generate sentences, we measured the time it took to generate 100 tokens long 100 times. The gated method took similar time regardless of the detoxifier(Figure~\ref{fig:exp_gated_detox_efficiency}).


\input{tab_efficiency}
% 메모리 효과적이에요
The larger the detoxifier, the better the performance. However, in the gated detoxifier, even a small detoxifier shows performance similar to that of a large detoxifier. Smaller detoxifiers use less memory and generate faster. After learning Experts and Anti-Experts of 124M number of parameters, we generated 100 text of 100 token length with DExperts and evaluated them. Gate Model's number of parameters is 110M. Table \ref{tab:exp_gated_detox_efficiency}



%
% Large-scale
%

\section{Large-scale Result}
In this section, we demonstrated that large-scale LM with Detoxifier degrade performance as small-scale did. Also We show that the gated detoxifier works well at large-scale. The human evaluation result is also similar to the automatic evaluation result.

\subsection{Automatic Evaluation Result}

\subsection{Human Evaluation Result}
% \include{tab_slightly_toxic_examples}
\include{tab_large_eval}

==> alg/alg_pseudo.tex <==
% \begin{algorithm}
% \caption{Gated Detoxifier}\label{alg:cap}
% \begin{algorithmic}
% \Require \\
% {
% \LM, \Comment{Lanugage model} \\
% \calD, \Comment{Detoxifier} \\
% \calG \Comment{Binary Toxic Classifier} \\
% }
% \State tokens = [ ]
% \While{$i \leq$ Len}
% \State probs = \LM(tokens)
% \State next = sample(probs)

%     \If{\calG(probs, next) \geq $0.5$}

%     \State probs = \calD(tokens, probs)
%     \State next = sample(probs)
% \EndIf
% \State tokens += next
% \EndWhile

% \end{algorithmic}
% \end{algorithm}


% \begin{lstlisting}
% function gated_detoxifier(LM, D, G):
%   tokens = []
%   for i = 1 .. max_length:
%     probs = LM(tokens)
%     next = sample(probs)

%     if G(probs, next) >= 0.5:
%       probs = D(tokens, probs)
%       next = sample(probs)
      
%     tokens += next
% \end{lstlisting}

==> table/tab_allexp.tex <==
\begin{table}[]
\begin{tabular}{l|lll|lll|lll|}
\cline{2-10}
                                          & \multicolumn{3}{l|}{sentiment}                                          & \multicolumn{3}{l|}{emotion}                                            & \multicolumn{3}{l|}{topic}                                              \\ \hline
\multicolumn{1}{|l|}{Model}               & \multicolumn{1}{l|}{Accuracy} & \multicolumn{1}{l|}{Toxicity} & Grammar & \multicolumn{1}{l|}{Accuracy} & \multicolumn{1}{l|}{Toxicity} & Grammar & \multicolumn{1}{l|}{Accuracy} & \multicolumn{1}{l|}{Toxicity} & Grammar \\ \hline
\multicolumn{1}{|l|}{GPT2-small}          & \multicolumn{1}{l|}{76.70}    & \multicolumn{1}{l|}{0.35}     & 95.05   & \multicolumn{1}{l|}{63.00}    & \multicolumn{1}{l|}{4.95}     & 94.10   & \multicolumn{1}{l|}{66.88}    & \multicolumn{1}{l|}{0.30}     & 79.23   \\ \hline
\multicolumn{1}{|l|}{DExperts(0.5)}       & \multicolumn{1}{l|}{71.80}    & \multicolumn{1}{l|}{0.35}     & 64.20   & \multicolumn{1}{l|}{45.00}    & \multicolumn{1}{l|}{1.92}     & 47.68   & \multicolumn{1}{l|}{60.12}    & \multicolumn{1}{l|}{0.08}     & 31.35   \\ \hline
\multicolumn{1}{|l|}{DExperts-Gated(0.5)} & \multicolumn{1}{l|}{77.50}    & \multicolumn{1}{l|}{0.00}     & 95.65   & \multicolumn{1}{l|}{63.50}    & \multicolumn{1}{l|}{1.30}     & 93.78   & \multicolumn{1}{l|}{66.67}    & \multicolumn{1}{l|}{0.08}     & 78.87   \\ \hline
\multicolumn{1}{|l|}{DExperts(1.0)}       & \multicolumn{1}{l|}{69.35}    & \multicolumn{1}{l|}{0.10}     & 47.10   & \multicolumn{1}{l|}{42.98}    & \multicolumn{1}{l|}{0.75}     & 33.78   & \multicolumn{1}{l|}{60.60}    & \multicolumn{1}{l|}{0.02}     & 31.07   \\ \hline
\multicolumn{1}{|l|}{DExperts-Gated(1.0)} & \multicolumn{1}{l|}{75.10}    & \multicolumn{1}{l|}{0.05}     & 95.85   & \multicolumn{1}{l|}{62.92}    & \multicolumn{1}{l|}{0.98}     & 93.98   & \multicolumn{1}{l|}{66.65}    & \multicolumn{1}{l|}{0.00}     & 79.00   \\ \hline
\multicolumn{1}{|l|}{GeDi(15)}            & \multicolumn{1}{l|}{74.95}    & \multicolumn{1}{l|}{0.05}     & 89.80   & \multicolumn{1}{l|}{57.98}    & \multicolumn{1}{l|}{0.13}     & 93.23   & \multicolumn{1}{l|}{66.87}    & \multicolumn{1}{l|}{0.02}     & 79.45   \\ \hline
\multicolumn{1}{|l|}{GeDi-Gated(15)}      & \multicolumn{1}{l|}{74.35}    & \multicolumn{1}{l|}{0.00}     & 94.45   & \multicolumn{1}{l|}{63.63}    & \multicolumn{1}{l|}{0.65}     & 93.73   & \multicolumn{1}{l|}{66.95}    & \multicolumn{1}{l|}{0.05}     & 78.75   \\ \hline
\multicolumn{1}{|l|}{GeDi(30)}            & \multicolumn{1}{l|}{74.50}    & \multicolumn{1}{l|}{0.00}     & 87.10   & \multicolumn{1}{l|}{56.30}    & \multicolumn{1}{l|}{0.00}     & 93.88   & \multicolumn{1}{l|}{66.70}    & \multicolumn{1}{l|}{0.05}     & 78.53   \\ \hline
\multicolumn{1}{|l|}{GeDi-Gated(30)}      & \multicolumn{1}{l|}{73.85}    & \multicolumn{1}{l|}{0.00}     & 94.75   & \multicolumn{1}{l|}{63.93}    & \multicolumn{1}{l|}{0.55}     & 92.92   & \multicolumn{1}{l|}{66.63}    & \multicolumn{1}{l|}{0.00}     & 78.53   \\ \hline
\multicolumn{1}{|l|}{PPLM}                & \multicolumn{1}{l|}{74.75}    & \multicolumn{1}{l|}{1.00}     & 46.95   & \multicolumn{1}{l|}{47.18}    & \multicolumn{1}{l|}{1.10}     & 44.40   & \multicolumn{1}{l|}{68.80}    & \multicolumn{1}{l|}{0.05}     & 26.63   \\ \hline
\multicolumn{1}{|l|}{PPLM-gated}          & \multicolumn{1}{l|}{80.45}    & \multicolumn{1}{l|}{0.15}     & 97.50   & \multicolumn{1}{l|}{65.65}    & \multicolumn{1}{l|}{2.00}     & 93.32   & \multicolumn{1}{l|}{66.72}    & \multicolumn{1}{l|}{0.07}     & 80.45   \\ \hline
\end{tabular}
\end{table}

==> table/tab_dataset.tex <==

\begin{table*}[ht]
\centering
\caption{Accuracy, Toxicity, Grammar average score per dataset } 
\begin{adjustbox}{width=1\textwidth}
\small
\begin{tabular}{l|lll|lll|lll|}
\cline{2-10}
                                          & \multicolumn{3}{l|}{sentiment}                                          & \multicolumn{3}{l|}{emotion}                                            & \multicolumn{3}{l|}{topic}                                              \\ \hline
\multicolumn{1}{|l|}{Model}               & \multicolumn{1}{l|}{Accuracy} & \multicolumn{1}{l|}{Toxicity} & Grammar & \multicolumn{1}{l|}{Accuracy} & \multicolumn{1}{l|}{Toxicity} & Grammar & \multicolumn{1}{l|}{Accuracy} & \multicolumn{1}{l|}{Toxicity} & Grammar \\ \hline
\multicolumn{1}{|l|}{GPT2-small}          & \multicolumn{1}{l|}{76.70}    & \multicolumn{1}{l|}{0.35}     & 95.05   & \multicolumn{1}{l|}{63.00}    & \multicolumn{1}{l|}{4.95}     & 94.10   & \multicolumn{1}{l|}{66.88}    & \multicolumn{1}{l|}{0.30}     & 79.23   \\ \hline
\multicolumn{1}{|l|}{DExperts(0.5)}       & \multicolumn{1}{l|}{71.80}    & \multicolumn{1}{l|}{0.35}     & 64.20   & \multicolumn{1}{l|}{45.00}    & \multicolumn{1}{l|}{1.92}     & 47.68   & \multicolumn{1}{l|}{60.12}    & \multicolumn{1}{l|}{0.08}     & 31.35   \\ \hline
\multicolumn{1}{|l|}{DExperts-Gated(0.5)} & \multicolumn{1}{l|}{77.50}    & \multicolumn{1}{l|}{0.00}     & 95.65   & \multicolumn{1}{l|}{63.50}    & \multicolumn{1}{l|}{1.30}     & 93.78   & \multicolumn{1}{l|}{66.67}    & \multicolumn{1}{l|}{0.08}     & 78.87   \\ \hline
\multicolumn{1}{|l|}{DExperts(1.0)}       & \multicolumn{1}{l|}{69.35}    & \multicolumn{1}{l|}{0.10}     & 47.10   & \multicolumn{1}{l|}{42.98}    & \multicolumn{1}{l|}{0.75}     & 33.78   & \multicolumn{1}{l|}{60.60}    & \multicolumn{1}{l|}{0.02}     & 31.07   \\ \hline
\multicolumn{1}{|l|}{DExperts-Gated(1.0)} & \multicolumn{1}{l|}{75.10}    & \multicolumn{1}{l|}{0.05}     & 95.85   & \multicolumn{1}{l|}{62.92}    & \multicolumn{1}{l|}{0.98}     & 93.98   & \multicolumn{1}{l|}{66.65}    & \multicolumn{1}{l|}{0.00}     & 79.00   \\ \hline
\multicolumn{1}{|l|}{GeDi(15)}            & \multicolumn{1}{l|}{74.95}    & \multicolumn{1}{l|}{0.05}     & 89.80   & \multicolumn{1}{l|}{57.98}    & \multicolumn{1}{l|}{0.13}     & 93.23   & \multicolumn{1}{l|}{66.87}    & \multicolumn{1}{l|}{0.02}     & 79.45   \\ \hline
\multicolumn{1}{|l|}{GeDi-Gated(15)}      & \multicolumn{1}{l|}{74.35}    & \multicolumn{1}{l|}{0.00}     & 94.45   & \multicolumn{1}{l|}{63.63}    & \multicolumn{1}{l|}{0.65}     & 93.73   & \multicolumn{1}{l|}{66.95}    & \multicolumn{1}{l|}{0.05}     & 78.75   \\ \hline
\multicolumn{1}{|l|}{GeDi(30)}            & \multicolumn{1}{l|}{74.50}    & \multicolumn{1}{l|}{0.00}     & 87.10   & \multicolumn{1}{l|}{56.30}    & \multicolumn{1}{l|}{0.00}     & 93.88   & \multicolumn{1}{l|}{66.70}    & \multicolumn{1}{l|}{0.05}     & 78.53   \\ \hline
\multicolumn{1}{|l|}{GeDi-Gated(30)}      & \multicolumn{1}{l|}{73.85}    & \multicolumn{1}{l|}{0.00}     & 94.75   & \multicolumn{1}{l|}{63.93}    & \multicolumn{1}{l|}{0.55}     & 92.92   & \multicolumn{1}{l|}{66.63}    & \multicolumn{1}{l|}{0.00}     & 78.53   \\ \hline
\multicolumn{1}{|l|}{PPLM}                & \multicolumn{1}{l|}{74.75}    & \multicolumn{1}{l|}{1.00}     & 46.95   & \multicolumn{1}{l|}{47.18}    & \multicolumn{1}{l|}{1.10}     & 44.40   & \multicolumn{1}{l|}{68.80}    & \multicolumn{1}{l|}{0.05}     & 26.63   \\ \hline
\multicolumn{1}{|l|}{PPLM-gated}          & \multicolumn{1}{l|}{80.45}    & \multicolumn{1}{l|}{0.15}     & 97.50   & \multicolumn{1}{l|}{65.65}    & \multicolumn{1}{l|}{2.00}     & 93.32   & \multicolumn{1}{l|}{66.72}    & \multicolumn{1}{l|}{0.07}     & 80.45   \\ \hline
\end{tabular}
\label{tab:topic_avg}
\end{adjustbox}
\end{table*} 

% \begin{table*}[ht]
% \centering
% \caption{Generation Speed comparison} 
% \begin{adjustbox}{width=0.5\textwidth}
% \small
% \begin{tabular}{ll}
% \hline
% \textbf{Model}                & \textbf{Generation Time} \\ \hline
% GPT2                          & 1000                     \\ \hline
% DExperts                      & 2500                     \\ 
% \textbf{Gated-DExperts(ours)} & \textbf{1700}            \\ \hline
% GeDi                          & 2100                     \\ 
% \textbf{Gated-GeDi(ours)}     & \textbf{1700}            \\ \hline
% \end{tabular}
% \end{adjustbox}
% \end{table*} 


==> table/tab_slightly_toxic_examples.tex <==

\begin{table}[t]
\caption{Slightly toxic examples generated by Fine-tuned small-scale LM} 
\begin{adjustbox}{width=0.47\textwidth}
\small
\begin{tabular}{l|l|l}
Topic    & Generated Example                                                                                                                             & Toxicity \\ \hline
politics & muslims and christians jailed on gay marriage law ...                                                                                         & 0.324    \\ \hline
negative & \begin{tabular}[c]{@{}l@{}}A very depressing restaurant.  It was very dirty, \\ I could have been in the back of a truck and ...\end{tabular} & 0.396    \\ \hline
love     & \begin{tabular}[c]{@{}l@{}}i feel like it wasn't a good look for a lady \\ because her skin was a mess\end{tabular}                           & 0.377   
\end{tabular}
\label{tab:slightly_toxic_generation}
\end{adjustbox}
\end{table}

